Computing Equilibria in Binary Networked Public Goods Games

Public goods games study the incentives of individuals to contribute to a public good and their behaviors in equilibria. In this paper, we examine a specific type of public goods game where players are networked and each has binary actions, and focus on the algorithmic aspects of such games. First, we show that checking the existence of a pure-strategy Nash equilibrium is NP-complete. We then identify tractable instances based on restrictions of either utility functions or of the underlying graphical structure. In certain cases, we also show that we can efficiently compute a socially optimal Nash equilibrium. Finally, we propose a heuristic approach for computing approximate equilibria in general binary networked public goods games, and experimentally demonstrate its effectiveness.

==> sections/algorithm.tex <==
%Since there may not exist PSNE even if the underlying graph $\mathcal{G}$ is complete. Additionally, by Theorem~\ref{thm-hard} we know checking the existence of PSNE in general is diffcult. 

\subsection{Games on Arbitrary Graphs}
We describe a heuristic algorithm to find an approximate PSNE for
a general BNPG.
An approximate PSNE is defined as follows:

\begin{defn}
    Given a heterogeneous BNPG, an approximate PSNE (i.e., \aPSNE) is an action profile $\ActionVec \in \SET{0, 1}^n$ such that:
	    \begin{equation*}
	           U_i(\Action{i}, \InvNum{i}{\ActionVec}) + \epsilon \ge U_i(1-\Action{i}, \InvNum{i}{\ActionVec})
	    \end{equation*}
	for all $i \in \V$.
\end{defn}


The heuristic algorithm consists of two subroutines.
The first one is termed as \textsc{Asynchronous-BR},
which is based on the idea of best-response dynamics.
In one iteration of \textsc{Asynchronous-BR}, each player will sequentially update her action with the best-response to the current action profile, in an asynchronous manner (i.e., later players can observe the actions of former players in the same iteration). 
The second subroutine is termed \textsc{Evolve}; it executes \textsc{Asynchronous-BR} \numEvo times and each execution generates an \aPSNE; finally \textsc{Evolve} picks the \aPSNE with the minimum $\epsilon$.
In this way, \textsc{Evolve} finds the approximate PSNE with the best quality (in items of $\epsilon$) through best-response dynamics. 
The pseudocodes of \textsc{Asynchronous-BR} and \textsc{Evolve}
are provided in the Appendix.
The heuristic algorithm is summarized in Algorithm~\ref{algo:heuristic}.  
The input \StopCond is the stopping criterion; the algorithm stops when the distance of two consecutive profiles (e.g., measured by some $\ell_p$ norm) is less than \StopCond or when the maximum number of iterations is exceeded.


\begin{algorithm}[ht]
	\caption{Heuristic to find \aPSNE}\label{algo:heuristic}
		\begin{algorithmic}[1]
			\State \textbf{Input}: $\numEvo$, $\StopCond$, $K$ \Comment{$B$: maximum number of iterations}
			\State Initialize: $d = M, i = 0$ \Comment{$M$: a large positive number}
			\State $\ActionVec \leftarrow $ random initializatioin
			\If{\ActionVec is a PSNE}
			    \State return \ActionVec
			\EndIf
			\While{$d \ge \StopCond$ and $i < B$}
			\State $i \leftarrow i + 1$
			\State $\ActionVec' \leftarrow$ \textsc{Evolve}($\ActionVec, \numEvo$) \Comment{run $\numEvo$ trials of the \textsc{Evolve} subroutine}
			\If{$\ActionVec'$ is a PSNE}
				\State return $\ActionVec'$
			\Else
				\State $d \leftarrow \Norm{\ActionVec' - \ActionVec}_p$ 
			\EndIf
			\EndWhile
			\State return $\ActionVec'$
		\end{algorithmic}
\end{algorithm}





% The second function called \textsc{maxEpsilon} is showed in Algorithm~\ref{algo:maxEpsilon}. Given an underlying graph $\mathcal{G}$ and a profile $\bm{x}$, if the profile is not a PSNE then Algorithm~\ref{algo:maxEpsilon} finds the maximum $\epsilon$ needed to make it a PSNE. Note that the loss functions $L_i$ in step $4$ are normalized so that $\epsilon \in [0,1]$. Intuitively, a profile $\bm{x}$ is closer to being a PSNE if the maximum epsilon associated with it is smaller. 


% For space limitation, a sketch of the heuristic algorithm to find $\epsilon$-PSNE is showed in Algorithm~\ref{algo:heuristic}:
% \begin{algorithm}[h]
% \caption{Heuristic to find $\epsilon$-PSNE}\label{algo:heuristic}
% \begin{algorithmic}[1]
% \State \textbf{Input}: $c_i, \lambda_i, g_i, \forall i=1,\cdots, n$, $\mathcal{G}, k$ and $\delta$
% \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}[h]
% \caption{Heuristic to find $\epsilon$-PSNE}\label{algo:heuristic}
% \begin{algorithmic}[1]
% \Function{isPSNE}{$\bm{x}, \mathcal{G}$}
% 	\State $flag=0$
% 	\For{$i=1, \cdots, n$}
% 		\If{$L_i(\bm{x}_i, n_i) > L_i(1 - \bm{x}_i, n_i)$} \Comment{$n_i = \sum_{j\in \mathcal{N}(i)}^{}{\bm{x}_j}$}
% 			$flag=1$
% 			\State break
% 		\EndIf
% 	\EndFor
% 	\If{$flag=0$}
% 		\State return True
% 	\Else
% 		\State return False
% 	\EndIf
% \EndFunction
% \\

% \Function{maxEpsilon}{$\bm{x}, \mathcal{G}$}
% 	\State $\epsilon=-\infty$
% 	\For{$i=1, \cdots, n$}
% 		% \State $n_i = \sum_{j\in \mathcal{N}(i)}^{}{\bm{x}_j}$
% 		\State $t = L_i(\bm{x}_i, n_i) > L_i(1 - \bm{x}_i, n_i)$
% 		\If{$t > 0$}
% 			\If{$t > \epsilon$}
% 				\State $\epsilon = t$
% 			\EndIf
% 		\EndIf
% 	\EndFor
% 	\State return $\epsilon$
% \EndFunction
% \\

% \Function{Evolve}{$\bm{x}, \mathcal{G}, k$}
% 	\State Initialize: $\bm{x}^\prime=\bm{0}, \epsilon^\prime=\infty$
% 	\For{$i=1, \cdots, k$}
% 		\State $\epsilon \leftarrow$ \Call{maxEpsilon}{$\bm{x}, \mathcal{G}$}
% 		\If{$\epsilon = -\infty$} \Comment{Found a PSNE}
% 			\State return $\bm{x}$
% 		\Else
% 			\If{$\epsilon < \epsilon^\prime$}
% 				\State $\epsilon^\prime = \epsilon$
% 				\State $\bm{x}^\prime=\bm{x}$
% 			\EndIf
% 		\EndIf
% 	\EndFor
% 	\State return $\bm{x}^\prime$
% \EndFunction
% \\

% \Function{Heuristic}{$\bm{x}, \mathcal{G}, k, \delta$}
% 	\State $\bm{x}^0=\bm{x}$
% 	\State $\bm{x}^1 \leftarrow$ \Call{Evolve}{$\bm{x}, \mathcal{G}, k$}
% 	\If{$L_i(\bm{x}^1_i, n_i)$}

% 	\EndIf
% 	\State
% % \State \While{}
% \EndFunction
% % \State \textbf{Input}: $c_i, \lambda_i, g_i, \forall i=1,\cdots, n$, $\mathcal{G}$, and $k$
% % \State Randomly initialize: $\bm{x}^{(0)}$
% \end{algorithmic}
% \end{algorithm}
